RandMSAugment: A Mixed-Sample Augmentation for Limited-Data Scenarios

The high costs of annotating large datasets suggests a need for effectively training CNNs with limited data, and data augmentation is a promising direction. We study foundational augmentation techniques, including Mixed Sample Data Augmentations (MSDAs) and a no-parameter variant of RandAugment termed Preset-RandAugment, in the fully supervised scenario. We observe that Preset-RandAugment excels in limited-data contexts while MSDAs are moderately effective. We show that low-level feature transforms play a pivotal role in this performance difference, postulate a new property of augmentations related to their data efficiency, and propose new ways to measure the diversity and realism of augmentations. Building on these insights, we introduce a novel augmentation technique called RandMSAugment that integrates complementary strengths of existing methods. RandMSAugment significantly outperforms the competition on CIFAR-100, STL-10, and Tiny-Imagenet. With very small training sets (4, 25, 100 samples/class), RandMSAugment achieves compelling performance gains between 4.1% and 6.75%. Even with more training data (500 samples/class) we improve performance by 1.03% to 2.47%. RandMSAugment does not require hyperparameter tuning, extra validation data, or cumbersome optimizations.

==> sec/misc.tex <==

\section{Differences with Automix Experiments}
\begin{enumerate}
    \item Use cosine annealing scheduler with some warm-ups. Since their method involves training an extra mix block and network head, which would be affected by a change in the scheduling, we didn't change this. 
    \item There was a slight difference in the mean std used for normalization.
    \item The default network size is WRN 28-8, we changed the architecture to match the one we use: WRN 28-10. However, the add thousands of extra parameters through the mix block and head networks. So we also use WRN-28-9 in order to match their parameters with that used in other methods more closely.
    \item Their batch size is 100, and number of epochs is 800. Ours is 64, and number of training epochs is 1342.
    \item Learning rate was 0.03.
    \item We use trainable\_params = sum(p.numel() for p in model.model.parameters() if p.requires\_grad)
to compute difference in number of trainable parameters. 
\item For validation and for testing they use the test set.
\item The store the best checkpoint upto the current training point. 
\item They report the median results over the last 10 epochs
\item They have 2 classification heads for each student and teacher: one is the usual classification head trained with the soft mixup loss, the other is a one-hot classificiation head (unaugmented samples or best predicted class?). They report the best among the 4 heads. 
\item 

\end{enumerate}


\begin{table}
    \centering
    \begin{tabular}{ccc|c}
        Network &  WRN 28-9 & WRN 28-10 & Preact-Resnet18\\
         Baseline &  29.613748 M & 36.54698 M & 11.268744 M \\
         Automix & 29.713353 M & 36.662761 M & 11.404497 M \\
         Difference & 99,605 & 115,781 & 135,753 \\
         \hline         
    \end{tabular}
    \caption{Automix uses about 100-116K more parameters more. Hence the comparison is not fair, even if methods use the same data, a model with higher number of parameters has more representation power.  }
    \label{tab:my_label}
\end{table}
The bi-level optimization in AutoMix \cite{zhu2020automix} is unstable when trained with limited data, as noted by the authors themselves. 

